The mother of all states of the kagome quantum antiferromagnet

Frustrated quantum magnets are a central theme in condensed matter physics due to the richness of their phase diagrams. They support a panoply of phases including various ordered states and topological phases. Yet, this problem has defied a solution for a long time due to the lack of controlled approximations which make it difficult to distinguish between competing phases. Here we report the discovery of a special quantum macroscopically degenerate point in the XXZ model on the spin-1/2 kagome quantum antiferromagnet for the ratio of Ising to antiferromagnetic transverse coupling Jz/J=-1/2. This point is proximate to many competing phases explaining the source of the complexity of the phase diagram. We identify five phases near this point including both spin-liquid and broken-symmetry phases and give evidence that the kagome Heisenberg antiferromagnet is close to a transition between two phases.

==> makefile <==
SHELL := /bin/bash
PROJECT=main_arxiv
TEX=pdflatex
BIBTEX=bibtex
BUILDTEX=$(PROJECT).tex

all:
	$(BIBTEX) $(BUILDTEX);                      \
	$(TEX) $(BUILDTEX);                      \
	for auxfile in $(wildcard *.aux); 	\
	do                                	\
		$(BIBTEX) `basename $$auxfile .aux`; \
	done;                                        \
	$(TEX) $(BUILDTEX);                         \
	$(TEX) $(BUILDTEX);                         
	
clean:
	rm -f *.log *.bak *.aux *.bbl *.blg *.idx *.toc *.out *~

